Capturing Label Distribution: A Case Study in NLI

We study estimating inherent human disagreement (annotation label distribution) in natural language inference task. Post-hoc smoothing of the predicted label distribution to match the expected label entropy is very effective. Such simple manipulation can reduce KL divergence by almost half, yet will not improve majority label prediction accuracy or learn label distributions. To this end, we introduce a small amount of examples with multiple references into training. We depart from the standard practice of collecting a single reference per each training example, and find that collecting multiple references can achieve better accuracy under the fixed annotation budget. Lastly, we provide rich analyses comparing these two methods for improving label distribution estimation.

==> tex/ethics.tex <==
\section*{Ethical Considerations}
This paper does not introduce new datasets and nor include demographic or identity characteristics in analysis. All our experiments are conducted on GPU computing resources, and it is manageable with a machine with four Quadro RTX 8000 graphics cards. In this paper, we focus on natural language inference (NLI). 
% NLI studies whether a hypothesis can be inferred from a premise, where both are a text sequence. 
This task can be applied to the fields where it requires the reasoning such as question answering and search engine. 
